Adding 32-bit Mode to the ACL2 Model of the x86 ISA

The ACL2 model of the x86 Instruction Set Architecture was built for the 64-bit mode of operation of the processor. This paper reports on our work to extend the model with support for 32-bit mode, recounting the salient aspects of this activity and identifying the ones that required the most work.

==> eptcsdata.tex <==
\providecommand{\firstpage}{77}
\providecommand{\publicationstatus}{Shilpi Goel and Matt Kaufmann (Eds.):\\
ACL2 Theorem Prover and its Applications (ACL2-2018)\\
EPTCS 280, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.280.6}{10.4204/EPTCS.280.6}}

